Expanding the Design Space of Computer Vision-based Interactive Systems for Group Dance Practice

Group dance, a sub-genre characterized by intricate motions made by a cohort of performers in tight synchronization, has a longstanding and culturally significant history and, in modern forms such as cheerleading, a broad base of current adherents. However, despite its popularity, learning group dance routines remains challenging. Based on the prior success of interactive systems to support individual dance learning, this paper argues that group dance settings are fertile ground for augmentation by interactive aids. To better understand these design opportunities, this paper presents a sequence of user-centered studies of and with amateur cheerleading troupes, spanning from the formative (interviews, observations) through the generative (an ideation workshop) to concept validation (technology probes and speed dating). The outcomes are a nuanced understanding of the lived practice of group dance learning, a set of interactive concepts to support those practices, and design directions derived from validating the proposed concepts. Through this empirical work, we expand the design space of interactive dance practice systems from the established context of single-user practice (primarily focused on gesture recognition) to a multi-user, group-based scenario focused on feedback and communication.

==> sections/03_ResearchOverview.tex <==

% Note: this section/file is currently excluded from the paper. 
In designing interactive systems for group dance contexts within HCI, we prioritized a human-centered approach to deeply understand Human-human Interactions(HHI) \cite{pritchard1988effects, weldon1993group}. This focus is essential, as comprehending the dynamics of group dance at a human level is fundamental to creating systems that effectively support and enhance these interactions. Our research began with a comprehensive literature review of 22 articles to establish the existing design space (Figure \ref{fig:researchOverview}-1). We then conducted a formative study, where observations and interviews with group dancers revealed 24 specific needs and pain points (Figure \ref{fig:researchOverview}-2). This insight guided a design ideation workshop with six designers, resulting in 55 innovative ideas, which we refined into 15 storyboards to articulate new design dimensions (Figure \ref{fig:researchOverview}-3). The final evaluation phase, using technology probes and speed dating workshops focused on RGB camera-based designs, tested these dimensions against potential user experiences (Figure \ref{fig:researchOverview}-4). This approach ensured that our expansion of the design space was not only theoretically sound but also deeply rooted in the real-world nuances of group dance practice.




% \begin{figure*}[]
%   \centering
%   \includegraphics[width=0.9\textwidth]{figures/existingDesignSpace.pdf}
%   \caption{Existing Design Space: }
%   \Description{}
%   \label{fig:existingDesignSpace}
% \end{figure*}

% \begin{figure}[]
%   \centering
%   \includegraphics[width=0.5\textwidth]{figures/expandedDesignSpace.pdf}
%   \caption{Expanded Design Space: }
%   \Description{}
%   \label{fig:expandedDesignSpace}
% \end{figure}

==> sections/99_Discussion_old.tex <==
%%% SECTION
\section{Discussion}
% 1. Analyze the effectiveness and feasibility of the design alternatives in addressing the identified user needs and pain points.
% 2. Reflect on the technical implementation of the real-time movement evaluation system and its integration into the co-design workshop.
% 3. Discuss the implications of the research outcomes and their potential impact on the field of human-computer interaction and cheerleading practice.
\subsection{Revisiting Established Design Spaces for Dance Interactive Systems}
%%%% REVISE THIS SECTION!!!
Existing interactive systems for dance learning focus primarily on assessing and assisting individual performance\cite{kim}, using technologies such as kinect\cite{kyan_approach_2015, marquardt_super_2012, anderson_youmove_2013}, augmented reality [REF], wearable device\cite{dias_pereira_dos_santos_lets_2017}, and mobile\cite{choi_dance_2021, lee_pose_2020} to deliver the evaluation results of solo movements. These systems may provide simple real-time feedback forms, or they may provide feedback through a video interface\cite{zhou_syncup_2021, riviere_capturing_2019} or report\cite{guo_dancevis_2022, guo_phycovis_2021} after the behavior. While these technologies provide sophisticated capabilities focused on the individual, they often fail to address the multifaceted needs of group dance dynamics.

Furthermore, despite the importance of providing rich, varied feedback in the suitable form at the right time \cite{trajkova_takes_2018, trajkova_e-ballet_2016}, existing systems are stuck in a relatively limited solution space, offering a relatively limited set of feedback types. In particular, while studies have presented guidance feedback \cite{anderson_youmove_2013, elsayed_cameraready_2021}, movement guidance must be addressed \cite{trajkova_takes_2018, kang_dancing_2023}. Many interactive systems have focused on providing corrective feedback through quantified metrics \cite{choi_dance_2021, kim_real-time_2018} instead of the other types of feedback \cite{raheb_hci_2016, gibbons_feedback_2004}. While there have been interactive systems for the real-time group dance context \cite{lee_cheerup_2023, zhu_zoombatogether_2023}, a more decadent design space must be explored and evaluated for group dance contexts such as cheerleading, where complex synchronization and interpersonal coordination are paramount. More existing research must be needed because these systems overlook essential factors such as timing, synchronization, and cohesion among group members. Our research aims to expand this solution space by investigating interactive systems that meet the complex requirements of group dance practice, providing correction and adaptive and nuanced feedback forms.

기존 연구에서는 다른 사람들의 상태를 보여줌으로써 나만 못하는 것이 아니라는 안심을 할 수 있다는 가능성에 대해서 보여주었다 \cite{zhu_zoombatogether_2023}. 하지만 기존 연구처럼 온라인에서 익명으로 그룹의 패널을 보여주는 것과는 다르게 실제 댄스 스튜디오에서는 더 복잡한 group dynamics가 존재한다.

% 아직도 해결 안된 것: guidance
% 기존 시스템과의 차이: 스켈레톤 시각화 -> defamiliarisation
% 기존 시스템을 다르게 활용: CO/DA 몸에서 소리 나는 시스템
% 추가적으로 발견한 것: pre-notice, group reflection, public feedback

% - augmented mirror는 아직까지 제약이 많다. 기존에는 움직임을 연습하고 평가하기 위해서 다양한 augmented mirror 컨셉이 제시되어 왔다 [REF]. 기존의 전통적인 댄스 스튜디오에서도 거울을 활용하여 동작을 연습한다 [REF]. 하지만 굉장히 빠르고 역동적인 동작을 하면서 augmented mirror에 나타나는 시각적 cue를 모두 활용하기란 쉽지 않다. 또한 치어리딩과 같이 공연을 최종 목적으로 하는 댄스 crew의 경우에는 언젠가는 거울 없이 연습을 해야하므로 모든 연습 과정에 있어서 적절하게 사용될 수 있는 방식은 아니다. 특히, 동작을 하는 실시간으로 피드백을 줄 때에는 추상적이고 은은하게 전체적인 컬러를 활용하여 피드백을 주는 것이 좋다. 그 외에는 auditory feedback을 통해서 혼선을 주지 않고 피드백을 줄 수 있는 방안을 강구하는 것이 좋다.
% - +스켈레톤 시각화는 생각보다 그렇게 효과적이지 않았음. 오히려 낯설게 보기가 마찬가지로 관찰되었는데 그게 댄스 연습에 있어서는 부정적인 영향을 보였다.
% - 우리는 피드백을 주는 타이밍이 3가지가 있을 수 있음을 밝혀냈다. 일반적으로 corrective feedback은 동작을 평가하고 주어야 하므로 동작이 끝난 후에 줄 수 있다. 하지만, 그 이외의 피드백은 동작이 틀리지 않았음에도 특정 동작을 하기 직전에 제공 될 수도 있고, 또는 동작을 하는 동시에 제공될 수도 있다.
% - 우리는 동작의 유사도와 정확도를 중심으로 다루었지만, temporal alignment와 관련해서는 비교적 덜 탐색되었다. 우리는 그룹 컨텍스트에서는 사람이 여러 명일 수록 같은 동작을 다른 박자에 시작하는 안무를 연습하기에 적합하며, temporal alignment와 관련된 디자인 스페이스에 대해서 더 탐색될 필요가 있다고 판단한다.
% - 또한, 그 이외에도 실제 치어리딩 연습에서는 1) 안무를 얼마나 외웠는지, 2) 전반적인 동작의 유사도는 얼마나 일치하는지, 그리고 3) 손 동작 또는 시선 처리와 같은 매우 작고 디테일한 동작을 얼마나 정확하게 하는지에 대해서 평가된다. 이는 동작의 평가에 있어서 실제 컨텍스트에 적용되기 위해서는 새로운 metric과 표현 방법의 가능성에 대해서 시사한다.
% - 그리고 AI는 사용자의 emotion을 덜 고려한다. AI가 만약에 음성을 통해서 피드백을 준다면 그 톤이 굉장히 중요하다 [REF]. 계속해서 같은 사람에게 같은 피드백을 반복해서 주게 된다면 주눅이 들 수도 있다. 이런 경우에는 instructors는 감정적으로 케어를 해주기도 하는데 AI는 그러한 맥락을 고려하기 힘들다. 댄스 스튜디오 내에서 연습으로 인해 crew의 만족도가 떨어지는 negative feedback을 막으려면, 동기부여를 위한 피드백들도 중요하다. gamification을 통해 선의의 경쟁 등의 요소로써 활용하여 그룹 내의 동기를 고취시키는 방안도 있다.
% - 그리고 여전히 guidance는 해결이 잘 되고 있지 않다. 연습을 보조하는 interactive system의 궁극적인 기능은 틀린 동작의 지적이 아니라, 맞는 동작으로의 guidance가 되어야 한다. 특히나, 그룹 컨텍스트에서 intensive한 동작까지 수반된다면 실시간으로 동작을 guidance 해주는 것이 쉽지 않다. in-depth interview 결과, 피드백은 간결하고 추상적이어야 한다. speed dating workshop에서 참가자들은 시스템이 제공한 결과에 대해서 설명이 된다면 더 신뢰할 수 있을 것이라고 응답했다. 이러한 동작을 guide 해주는 문제가 잘 해결된다면,  사용자들의 시스템에 대한 신뢰도 또한 올라 갈 것으로 기대된다.


\subsection{Unveiling Design Space in Group Dance Practice Contexts}
We have identified the concept of group reflection and the new element of public or private that can be considered in interactive systems for dance practice. We propose the concept of group reflection as reflective feedback that allows the group to reflect on their group movements rather than correcting them \cite{raheb_hci_2016}. In particular, we have identified an expansion of the design space of existing body-generated sound systems. Traditionally, these systems have been utilized primarily for improvisational dance \cite{francoise_coda_2022}. Utilizing these systems for personal dance practice can be ambiguous for self-reflection. However, especially in group synchronized dance, where synchronization of movements is essential, it is possible to reflect on the synchronization of the current group's movements by seeing if everyone has generated sounds that are in sync. We also saw the potential to support group reflective practice by overlaying each other's skeletons, similar to how we practice in real life (lined up in front of a mirror).

Furthermore, we found that in the context of group dance practice, there is an additional factor that has been relatively little considered by previous studies: public or private feedback \cite{trajkova_takes_2018, raheb_hci_2016, raheb_dance_2019}. There is a potential concern that publicly giving feedback to a specific person repeatedly could lead to stress due to social pressure. On the other hand, public feedback can catalyze other coworkers to learn what they are doing wrong and work harder on their practice. It can also positively impact peers, as they can learn from each other's feedback and reflect on their practice or help their peers practice. Private feedback can be used if all members need to receive different feedback in parallel or to reduce social pressure. However, private feedback can also negatively affect motivation and commitment to practice since only the wrong person knows what they did wrong. 


\subsection{Design Considerations of Vision-based Interactive System for Group Dance Practice}
Using vision-based dance evaluation systems in group dance practice requires several considerations. To make such a vision-based interactive system usable in practice according to human-centered AI design guidelines, we need to 1) set initial user expectations well and 2) allow users to act appropriately when the system fails \cite{amershi_guidelines_2019}. For initial user expectations, it is essential to specify what the system can currently do (which body parts and how many people can be tracked, and that tracking may not work well if each other's bodies are occluded) and to provide a session for users to try it out early on so that expectations and trust can be adequately established. In particular, for multi-person pose estimation, it is necessary to specify the range that the camera can recognize to ensure that all dancers are present in the field of view and to preprocess the pose estimation results so that they are not distorted by spatial problems \cite{guo_phycovis_2021}. It is also important to successfully accomplish relatively simple tasks, such as robust tracking of static bodies, to overcome user frustration and trust in the system \cite{baughan_mixed-methods_2023}. 

In addition, there are additional user experience considerations when using these interactives. When utilizing equipment such as augmented mirrors, consideration should be given to not being distracted by the visual information that appears in the mirror \cite{trajkova_takes_2018, dearborn_mirror_2006}. In particular, real-time visual information may not be appropriate in group dance genres involving intensive movement, such as cheerleading. For example, visualizing a delayed skeleton or avatar can be a positive experience in the creative process of improvised dance, providing a new sense of self. However, in a system that can assist in practicing and evaluating movements, a dancer may need clarification on their movements and the delayed skeleton \cite{zhou_here_2023}. In other words, the suitable modality, feedback frequency, and feedback timing must be determined for the context of the exercise \cite{trajkova_takes_2018, wulf_frequent_1998}. In addition to selecting the system, parameters such as the system's sensitivity must also be adjustable by the user, depending on the level of the dancer or the difficulty of the movement \cite{magill_influence_1994}. Furthermore, some respondents used the analogy of a karaoke machine and said that a system cannot completely replace an instructor. Given these user expectations, the role of such interactive systems in dance studios should be considered. 

Giving feedback in a group context impacts group dynamics and creates social interaction. For example, group reflection has the potential to create cooperation to keep everyone on track, but revealing quantified metrics can create competition. This is similar to the view of competition versus cooperation within a group \cite{deutsch_cooperation_2011}. However, public feedback does not always encourage competition among certain users, nor does private feedback positively relieve psychological pressure, and competition is not necessarily a negative factor within a dance studio \cite{dimenichi_power_2015}. Therefore, while there is no correct answer to how to give feedback to dancers, and the characteristics of the dancers or the level of their movements should be considered \cite{magill_influence_1994}, we propose that the characteristics and context of the group should also be considered necessary. AI is still limited in reflecting complex and ambiguous contextual information from the real world, such as the dynamics of the group's characteristics \cite{yang_human-centered_2021}. The role of these interactive systems in the group context needs to be clarified by humans to avoid social confusion, such as the ambiguity of the instructor's role. Therefore, users must be able to select and intervene directly with the system according to the practice period or the current group context. 

%그룹의 특성에 따라서 어떠한 인터랙션이 생길지는 인간의 복잡한 맥락을 파악해야하기에 AI가 판단하기 어렵다. 하지만 온라인 컨텍스트가 아닌 실제 댄스 스튜디오 컨텍스트에서 실시간으로 public하게 피드백을 받게 되면 누가 얼마나 잘하고 못하는지 특정될 수 밖에 없다. 특히, 이전 연구\cite{zhu_zoombatogether_2023}에서 제기한 컨텍스트와 반대로 다른 동료들은 모두 잘하는데 한 사람만 못하는 경우가 있다면 그런 경우에서는 심리적으로 위축되기가 쉽다.

\begin{figure}[]
  \centering
  \includegraphics[width=0.7\textwidth]{figures/dancers-in-the-loop.pdf}
  \caption{Dancers-in-the-Loop: It represents the relationship between the dance studio's instructor, student, and AI system. The inverted triangle depicts the role of the AI system as an auxiliary tool, never as an equal to the dancers.}
  \Description{}
  \label{fig:dancersInTheLoop}
\end{figure}


\subsection{Dancers-in-the-Loop: The Role and Use of Interactive AI System for Group Dance Practice}
In this study, we wanted to evaluate the design space of systems easily accessible in a real-world context, so we focused on vision-based systems. In addition to that, it is necessary to clearly understand the relationship between the instructor, student, and AI system to use Interactive AI systems that support dance in any form in a dance studio. We propose the concept of Dancers-in-the-Loop for this purpose (Figure \ref{fig:dancersInTheLoop}). Dancers-in-the-Loop is a conceptual model of the relationship between dancers and the intelligence of AI within a dance studio, from a systemic perspective, where they can interact with each other and utilize AI effectively in the long run. As shown in Figure 0, the conceptual model consists of an outer and inner loop, and each element (instructor, student, and AI) interacts with the other. 

The outer loop describes how AI is supportive in the dance studio (Figure \ref{fig:dancersInTheLoop}A-C). A) First, the AI system captures, analyzes, and evaluates the student's body movements; B) The evaluation results are then sent to the instructor to help the instructor guide the practice; C) The instructor leading the dance studio decides how the results should be communicated to the students and what impact they can have and communicates them appropriately to the students. The inner loop describes how the dancers interact with the AI system (Figure \ref{fig:dancersInTheLoop}D-F). D) The instructor selects the appropriate interactive AI system based on the characteristics of the group, the timing of the exercise, and the current context of the exercise; E) Students practice with each other and receive feedback from the AI system; and F) the instructor can monitor how students are utilizing the system and intervene to replace it with a more appropriate system or adjust parameters such as assessment sensitivity. In step F, the instructor does not necessarily need to intervene in the system but rather the person who is temporarily leading the student group exercise.

Ultimately, when an interactive system is introduced inside a dance studio, the long-term impact it will have on the dance studio must be determined by the instructor and students, taking into account the characteristics of the group. Although the instructor's decision may seem prominent in the presented conceptual model, the interaction between the instructor and the student (Figure \ref{fig:dancersInTheLoop}C \& E) is essential. The student should be able to help the instructor make judgments and decisions, and the instructor should ensure that the student does not lose motivation in the exercises. In the long run, the instructor and student should work together to create a virtuous cycle for the entire amateur dance crew, including the dance studio. The system should not be utilized solely for the short-term and fragmented goal of improving the accuracy and similarity of efficient movements. Obsessing over short-term performance gains can harm the organization in the long run. These interactive systems can help dance studios keep members motivated in the long run.

\begin{figure}[]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/studentClubSystem.pdf}
  \caption{Systemic Approach to Student Dance Club: To understand the purpose and impact of an interactive system for group dance practice, we should take a systems approach. University student performance clubs go through cycles: A) Practice can be challenging, especially in synchronized dance. B) After overcoming this, they achieve high-quality performances and satisfaction. C) This motivates further practice. D) However, intense practice can lead to dissatisfaction. E) Social pressure plays a role in poor practice. Interactive AI systems must address these dynamics while improving movements efficiently. Neglecting social aspects could lead to short-term gains but long-term dissatisfaction. Consideration of the broader group impact is crucial.}
  \Description{}
  \label{fig:studentClubSystem}
\end{figure}

\subsection{Beyond Dance Studio: The Role of Interactive Systems from a System Perspective}
To better understand the ultimate purpose and potential impact of an interactive system that aids in group dance practice, we need to take a systems approach \cite{yildirim_how_2022}. If we look at the system of university students' performance clubs (Figure \ref{fig:studentClubSystem}), A) they usually practice for a specific performance (university, external, or their own). Practicing is not always a fun process, especially in the case of synchronized dance, where everyone has to do the same movements simultaneously, with no room for individuality or creativity. Sometimes, this process can feel tedious and exhausting. B) However, once they overcome this practice process, they can give a very high-quality performance, which gives them a sense of satisfaction and accomplishment. C) This motivates them to go through the repetitive, sometimes boring, and arduous process of practicing again. D) However, if the practice process becomes too intense, the opposite happens: they become less satisfied with the club activity. This creates a negative cycle of not practicing as hard, lowering the quality of the performance, and further decreasing satisfaction. 

One factor contributing to poor practice is social pressure in group contexts [ref]. Therefore, E) Interactive AI systems that support practice must be designed and utilized to consider these social dynamics while still doing what they should do: evaluate movements and help improve them more efficiently. Otherwise, it is easy to create a vicious circle in which any interactive system may actually improve movement faster in the short term, but in the long term, it may lead to less satisfaction with the club. To introduce such an Interactive AI system in a real dance studio, its impact must be considered, especially the social dynamics in a group context, which has not been considered much in existing work. In addition, even if an interactive system seems to solve a short-term problem, it may have adverse effects in the long run, such as the wicked problem \cite{berger_wicked_2017}, where it is difficult to know the impact of a larger group interacting with the system than in a one-to-one interaction.


%%%SECTION


==> sections/99_Results.tex <==
%%% SECTION
\section{Results}
% 1. Reflect on the findings from the user needs identification phase, highlighting the pain points and challenges identified through the interviews.
% 2. Discuss the outcomes of the co-design workshop, including the design alternatives proposed by the participants.
% 3. Reflect on the feedback and reactions of the cheerleaders and designers during the workshop.
%%%%%%
Since our overall research has focused on exploring and expanding a design space for vision-based interactive systems in group dance contexts, we summarize the results of evaluating this design space through technology and speed dating workshops. The lead author utilized thematic analysis methods to analyze and interpret what was discussed at the workshops \cite{braun_using_2006, hsieh_three_2005}.

%% This is subsection of Technology Probe
\subsection{Technology Probe Workshop Results}

% \begin{figure*}[]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/technologyProbeInsight1.pdf}
%   \caption{Technology Probe Table 1}
%   \Description{}
%   \label{tab:technologyProbeTable1}
% \end{figure*}

% \begin{figure*}[]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/technologyProbeInsight2.pdf}
%   \caption{Technology Probe Table 2}
%   \Description{}
%   \label{tab:technologyProbeTable2}
% \end{figure*}


\subsubsection{Initial Expectation:}
Participants had initial expectations of the system before trying it out. Some participants expected the AI system to provide consistent and objective ratings. "\textit{Sometimes one instructor thinks it's right and another thinks it's wrong, so I think this system would be an objective and accurate assessment.} (P1)" There was also an expectation that the cheerleading choreography would track detailed body parts (hand movements, head turns, etc.) that are traditionally difficult to see with the human eye. "\textit{When we're practicing detailed movements, we're checking a lot of hand gestures, like turning our heads to each other, so I think there was an expectation that those things would be tracked.} (P2)"

\subsubsection{Initial Test:}
Participants were initially free to test the technology's challenges and opportunities. They tested how accurately and quickly the system captured their bodies. In particular, they focused on movements that are typically utilized in cheerleading and tested how well it tracked them when they performed occlusive or vigorous movements. "\textit{I was curious about how far the skeleton was tracked, so I wanted to see if wrists and hands were tracked as well, to see how well it would recognize the body when turning around.} (P7)" They also tested the system by matching movements to each other and making small body movements to see how sensitive the system is to assessing the similarity of movements. "\textit{Since the system is measuring similarity between people, I wanted to get a little bit of a baseline of what it considers to be similar.} (P7)"

\subsubsection{Critique:}
Participants criticized the vision-based technology for its lack of real-world use in a dance studio. In particular, P6 mentioned that the camera's recognition speed is slightly delayed, which is confusing because it doesn't match your movements and the sound of your footsteps. P2 also pointed out that the camera's field of view is too narrow to recognize multiple people. In addition, another participant pointed out that the narrow-angle of view forces people to stand close to each other, and when performing vigorous movements such as cheerleading, body parts overlap, and tracking becomes difficult at that moment. "\textit{I think it would be better to use a wide-angle camera or something like that, because if we're all crammed together on a small screen, our bodies might overlap.} (P7)" One participant also criticized the limitations of 2D tracking, saying that even when the system thinks the movements are the same, they may actually be slightly different. "\textit{When we actually showed it, it felt a little out of order because we weren't matching the shape (the skeleton), we were matching the behavior (the body).} (P6)"

In addition to the vision-based pose evaluation system, some participants criticized the augmented mirror and its visual effects. P6 said that in the third probe (Figure \ref{fig:techProbeMerge}C), it was difficult to focus on other participants' skeletons and pay attention to their own movements, and P4 said that it was difficult to know if the movements were correct because the skeletons of other people were different from their actual body shapes. In addition, some participants said that in the fifth probe (Figure \ref{fig:techProbeMerge}E), the visual effects actually covered the mirror, which had the negative effect of distracting them. "\textit{I don't really see much of a difference, and I think it's more distracting to have to watch the motion and see the background change underneath.} (P4)"

\subsubsection{Suggestion:}
Participants provided several suggestions for the use of the technology in the context of real-world group dance practice. First, there were suggestions for improving the limitations of the pose tracking technology. P7 suggested that due to the limitations of the current 2D-based tracking technology, depth should also be measured, or a multi-view would be needed to evaluate cheerleading movements more rigorously. In addition, some participants wanted more control over the system. They wanted to adjust the sensitivity with which the system calculates pose similarity and set the duration (window size) for which feedback is provided if it is discrete. They felt that the system's settings should be different depending on the context of the practice. "\textit{I think if you make the system a little more sensitive when practicing the basics initially, the psychological pressure will make you work harder.} (P9)"

There were also responses about how the provided technology could be used differently in a dance studio: P6 said that it would be suitable for demonstrating and explaining the mechanics of the joints in a cheerleading move rather than for assessment purposes. "\textit{If the instructor has a skeleton visualization and says that the joints of the body follow this route, I think it's a little bit more intuitive to show how the body should move and the mechanism of the joints and stuff like that.} (P6)"

Participants also responded to how reliable these systems would be in practice in a dance studio. P9 said that the initial experience with the system would be important. In particular, P1 said they would naturally trust it when it showed them how their body was being captured, like a skeleton visualization, or when they saw the scores change in real time. Despite this, several participants said they did not fully trust the system. P6 and P7 felt that the systems were similar to the machines that rate songs at karaoke and that they would never fully replace human motion assessment.
%P7 said that he could see these systems being utilized to assist instructors in leading exercises.

% \begin{figure*}[]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/SpeedDatingInsight1.pdf}
%   \caption{Speed Dating Table 1}
%   \Description{}
%   \label{tab:speedDatingTable1}
% \end{figure*}

% \begin{figure*}[]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figures/SpeedDatingInsight2.pdf}
%   \caption{Speed Dating Table 2}
%   \Description{}
%   \label{tab:speedDatingTable2}
% \end{figure*}

%% This is a subsection of Speed Dating
\subsection{Speed Dating Workshop Results}
\subsubsection{Reflections on the Design Space for General Practice Applications}
\textbf{Augmented Mirror with Visual Cues:}
Participants discussed how the visualizations provided through the augmented mirror would be experienced in actual practice. Some participants felt that the visualizations provided through the mirror were distracting and took away from the role of the mirror. "It was a bit distracting. I don't know if it's used for games and stuff like that, but other than that, I don't think it's appropriate for a training situation. (P4)" P9 said that providing real-time visual feedback should be subtle enough to be perceived by squinting. In addition, P7 believes that those who can fully absorb the information provided by the mirror during intensive movement are already skilled enough not to need such an auxiliary system. He also believes that different systems are needed at different times of practice. "I think that someone who can check themselves by looking at the visual information in the mirror at that moment while running is already somewhat skilled in itself. (P7)" Besides, university cheerleading crews usually practice for performance. Other participants said that the closer they practice to the performance, the more they have to practice without mirrors and that visual aids are not very helpful. "At the end of the day, the performance itself is done in a situation with no visual support, so I don't think visuals will be very helpful at some point. (P6)" P2\&P3 said that auditory feedback would be relatively suitable for real-time feedback.

\textbf{Discrete Feedback vs Continuous Feedback:}
Participants discussed whether feedback should be provided continuously or discretely. Generally, when feedback was provided continuously, it was presented through a score (0 to 100) or color (0 to 255) to provide a more precise indication of the similarity of actions. On the other hand, discrete feedback was presented in five bins (Excellent-Good-Fair-Poor-Bad) to give a rough idea of the similarity of behaviors. P4 and P6 felt that individualized feedback was not really constructive because it seemed to say that only their movements in that moment were correct. P9 felt that the continuous feedback was more reliable and that the more precisely they could assess the similarity of the movements, the more reliable the system would be in practice, as it is vital in cheerleading to match each other's movements completely.

\textbf{Feedback Timing:}
Participants also broke down the timing of when feedback can be delivered to dancers. Typically, corrective feedback is given immediately after an incorrect movement, but there was also discussion of feedback given before or at the same time as a movement, even when the movement was not incorrect. In terms of feedback before performing a particular movement, P9 said that being told to push through a physically challenging section of the movement would fire her up. Another participant said that if she repeatedly got a certain section wrong, giving her guidance on what to do or shouting at her to focus on that section would make her more tense and focused (P1). In addition, one participant said that it would be helpful to be told the beat one after the other, especially if they were starting the movements sequentially. "I have friends who can't count the beats, so I think it would be good to have a reference for them so that if they miss something like that, they can now count the beats with a blinking time or something like that so that they can count the beats themselves. (P7)"


\textbf{Evaluation Metrics:}
The participants elaborated on the more critical information that should be conveyed to the dancers than the actual cheerleading practice situation. P4 mentioned that it is not very meaningful to point out someone who made a move wrong or only to communicate the score, but it is essential to communicate how to improve the move. In addition, P7 suggested the possibility of a new dance evaluation metric, not just calculating pose similarity or temporal alignment, but something evaluated sequentially in a practice session from a macro perspective. "I think it's a little less intuitive to have a score for each body part... In the training process, it's more like 'let's match the movements!' rather than 'let's train the arms!' I think it would be nice to have a score for each training process... Some points for memorizing the choreography, some points for matching the movements, some points for detailed movement... (P7)"


\subsubsection{Reflections on Design Space for Group-Specific Applications} 
\textbf{Group Reflection:}
The participants discussed their experiences with reflective feedback in cheerleading practice involving group rather than individual reflection. In particular, P6 and P7 mentioned that the concept of generating sounds with body movements to match the similarity of their movements through sound (Figure \ref{fig:teaser}E) was similar to how they use footsteps to check the beat in actual practice. In particular, some participants hoped that this concept would encourage them to collaborate with each other during practice. "\textit{I think it would be good because it would give us a small pleasure to match the sound, and it would give us a sense of cooperation to try to match it together.} (P4\&P6)" Regarding the concept of overlaying each other's body skeletons (Figure \ref{fig:teaser}F), one participant said that it was similar to the practice of wearing colored bracelets while standing in a line to match movements in real practice. "\textit{Like we actually practice with colored bracelets, I think if we have our own skeleton color, we can recognize it a little bit better.} (P2)"

\textbf{Public Feedback vs Private Feedback:}
Participants discussed receiving feedback publicly versus privately in group practice situations. P1, P5, and P6 said that they would feel stressed if they received feedback publicly in front of others that they were constantly doing poorly. On the other hand, some participants said that public feedback actually made them feel more socially tense. "\textit{I think it's really effective if you're motivated, but if you're not, I think you'll ignore private feedback.} (P1)"; "\textit{I think if we all listen to someone's feedback together, we can point out what they're doing wrong, so I think we need to know what we're doing wrong.} (P3\&P4)"

\subsubsection{Potential Challenges of Interactive Systems in Dance Studios}
\textbf{Quantified Evaluation Results:}
Participants mentioned the quantitative metrics that the system provides after evaluating their behavior. P1 said that these quantitative indicators gave him confidence in the system. On the other hand, some other participants were concerned that these quantitative metrics would hurt the group atmosphere. "\textit{I'm not sure why there's a score... The whole point of using a system like this is to improve something that's a little bit wrong, to make it better, not to see who's better...} (P4)"; "\textit{I'm comfortable with vague criteria, but I think it would bother me if my friend next to me got a 75 and I only got a 74.} (P6)"; "\textit{I think cheerleading is all about making the same moves together, so I don't think we need to break down who's good and who's not.} (P7)" In this regard, P7 believes that objective metrics such as grades should be passed through the instructor to the student as much as possible.

\textbf{Impact on Group Dynamics:}
Participants were concerned about the potential impact the system could have on group dynamics. Participants were concerned that the system could confuse the role of the instructor: "\textit{I think there could be cases where the instructor gives feedback that the behavior is wrong, but the students rebel because the AI says their behavior is right.} (P7)"; "\textit{I think there could be cases where the system and the instructor disagree. Since the behavior-matching process is centered around the instructor, who is also the crew's president, I think the instructor's opinion should come first.} (P1, P2)" Additionally, P8 mentioned possibly taking on an unwanted role. "\textit{In a small group context, if the system says I'm the best at something, I feel like I have to lead an exercise even if I don't want to lead the group.} (P8)"


\subsubsection{Potential Opportunities of Interactive Systems in Dance Studios}
\textbf{Purpose, Role, Use:}
Participants discussed how and for what purposes such a system could be utilized within a dance studio. Some participants mentioned that such a system could be used to set common goals and could be utilized for evaluation purposes. "\textit{I feel like we're more motivated to get it right.} (P7)"; "\textit{I think we'll practice movements a few times amongst ourselves and then use the system as a final evaluation.} (P2\&P3)" Participants also mentioned the need for the system to be selected and adapted to consider the group's characteristics and the practice period. "\textit{For example, it's okay if the music is interrupted when we're trying to figure out the moves together, but at the beginning, we don't know the choreography very well, so we're taught through skeleton visualization...  I think a different system should be used for each stage of learning.} (P4)" In addition, P9 noted that the choice of system should be considered in relation to the characteristics of the group. "\textit{I think it would be a lot of fun to use this as a game, like a good-natured competition, but I think you'd have to use it carefully depending on the group's disposition.} (P9)"

P7 also mentioned that such a system would serve as a tool to assist the instructor. He mentioned the process and dilemma of preparing these amateur student dance crews to perform and noted that balancing the use of these interactive systems is essential. "\textit{In the end, we practice for performance, but the higher the performance quality, the harder it is to practice and the less satisfied we are with the club. Since we are amateur students, we can be divided into those who want to enjoy club activities and those who want to make a great performance. It would be better if the characteristics and diversity of these amateur groups could be considered and used appropriately.} (P7)"

\textbf{Repurpose and Suggestion:}
Participants offered other suggestions for repurposing the system, particularly P7, noting that the concept of making sounds through the body could be utilized in choreography where the same movement is initiated on different beats. "\textit{I think if you use this system, even if you close your eyes, you can tell if you start the movement on the right beat.} (P7)" P7 also mentioned that it might be better to set a threshold for the score, showing only pass or fail depending on the context. "\textit{If the dancer crosses the threshold, the score is passed and the dancer is simply informed of the pass, and if the dancer fails, the detailed score is given to the instructor so that they can refer to it in their practice.} (P7)"

